Auditable Ledger Snapshot for Non-Repudiable Cross-Blockchain Communication

Blockchain interoperability is increasingly recognized as the centerpiece for robust interactions among decentralized services. Blockchain ledgers are generally tamper-proof and thus enforce non-repudiation for transactions recorded within the same network. However, such a guarantee does not hold for cross-blockchain transactions. When disruptions occur due to malicious activities or system failures within one blockchain network, foreign networks can take advantage by denying legitimate claims or mounting fraudulent liabilities against the defenseless network. In response, this paper introduces InterSnap, a novel blockchain snapshot archival methodology, for enabling auditability of crossblockchain transactions, enforcing non-repudiation. InterSnap introduces cross-chain transaction receipts that ensure their irrefutability. Snapshots of ledger data along with these receipts are utilized as non-repudiable proof of bilateral agreements among different networks. InterSnap enhances system resilience through a distributed snapshot generation process, need-based snapshot scheduling process, and archival storage and sharing via decentralized platforms. Through a prototype implementation based on Hyperledger Fabric, we conducted experiments using on-premise machines, AWS public cloud instances, as well as a private cloud infrastructure. We establish that InterSnap can recover from malicious attacks while preserving crosschain transaction receipts. Additionally, our proposed solution demonstrates adaptability to increasing loads while securely transferring snapshot archives with minimal overhead.

==> Main_Matter/decentralized_Interoperability.tex <==
\label{sec:decentralized_Interoperability}
Interoperability is the ability of computer systems or software to interact and exchange information. It is the ability of the networks to communicate with each other by sending and receiving signals, messages, data, tokens, etc. Major decentralized systems such as blockchains are mostly soloed; one blockchain can not interact with one another. This makes most blockchains incompatible with each other. However, there are a number of blockchains in existence, each with its unique properties. One system could be ideal for trade finance, while another is used for international payments, and another one ensures regulatory compliance. There must be a way for all these networks to talk to each other to intercommunicate as a whole. This paves the path for interoperability. The goal of interoperability is to make decentralized systems more compatible with one another and to allow their integration into existing systems. 
\par In the context of blockchain technology, interoperability refers to the exchange of data between blockchain networks. Such data exchange may either include the replication of data from one blockchain to another or the execution of functions conditional to information that was revealed on another blockchain. Without this interoperability, it would be difficult for organizations to utilize blockchain technology because they need access to an unlimited number of independent parties rather than just one centralized authority. It helps in getting rid of intermediaries and third parties. Organizations can use decentralized interoperability to track data and assets across disparate systems while providing immutability. Interoperability is essential because it allows different systems to coexist in a world where their data can be exchanged. It also enables different types of transactions on blockchain networks, like those with smart contracts or confidential transactions, to take place simultaneously with the presence of all parties. 

However, the process of blockchain interoperability is highly restricted at present. Blockchains currently cannot directly query external information. How to securely transfer data from one blockchain conforming to the consensus rules, satisfying the user’s policy, aligning to the inherent immutability of blockchains, and maintaining the security and privacy aspects are some of the significant challenges in the current situation.

==> Main_Matter/discussion.tex <==
\notebluerw{
While \ours is implemented using Hyperledger Fabric and Hyperledger Cacti, its architectural design is conceptually extensible to other interoperability frameworks such as Cosmos IBC \cite{kwon2019cosmos}, Chainlink CCIP \cite{breidenbach2021chainlink}, or Polkadot XCMP \cite{wood2016polkadot} For example, in Cosmos the SDK includes a native snapshot mechanism known as state sync, which is used primarily for efficient node synchronization. These snapshots capture the complete application state at a particular block height and are served in compressed chunks to new nodes joining the network. In the Cosmos IBC protocol cross-chain communication relies on proofs over Tendermint \cite{buchman2016tendermint} consensus. The endorsement logic in \ours could be replaced with IBC proofs of commitment (at Merkle root of the state change). Similarly, in Chainlink CCIP, trusted oracle signatures could substitute for Fabric’s endorsements to establish transaction validity. In Polkadot XCMP, snapshot generation could be integrated within the relay chain, leveraging its message exchange framework to enforce snapshot exchange. We plan to explore the adaptability of \ours on these interoperability protocols in a future work.
% While \ours is implemented using Hyperledger Fabric and Hyperledger Cacti, its architectural design is conceptually extensible to other interoperability frameworks such as Cosmos IBC, Chainlink CCIP, or Polkadot XCMP. For example, in Cosmos the SDK includes a native snapshot mechanism known as state sync, which is used primarily for efficient node synchronization. These snapshots capture the complete application state at a particular block height and are served in compressed chunks to new nodes joining the network. In the Cosmos IBC protocol cross-chain communication relies on proofs over Tendermint consensus. The endorsement logic in \ours could be replaced with IBC proofs of commitment (at Merkle root of the state change). Similarly, in Chainlink CCIP, trusted oracle signatures could substitute for Fabric’s endorsements to establish transaction validity. In Polkadot XCMP, snapshot generation could be integrated within the relay chain, leveraging its message exchange framework to enforce snapshot exchange. We plan to explore the adaptability of \ours on these interoperability protocols in a future work.
}

==> Main_Matter/relatedwork_lowoverhead.tex <==
\label{sec:relatedwork_lowoverhead}
Increasing data and resource usage for blockchain is a major concern. Ethereum, for example, the data size has reached approximately 1200 GB \cite{ycharts} by the end of November 2023. A similar concern \cite {hlc}, is highlighted by Hyperledger Labs, one of the most mature permisioned blockchain systems, in the present day.
The consistent growth of ledger heights also causes high memory consumption ~\cite{zamani2018rapidchain,wang2019monoxide,carminati2018confidential}, and slow bootstrapping of new peers \cite{xu2018cub,chepurnoy2016rollerchain}. 
An alternative less resource-intensive process can be used to initialize a new joiner using a snapshot \cite{hlfledgersnapshot,hlf}. \notebg{Are we suddenly motivating the use of snapshots here? If so it has to be done in intro, not related work. } 
A few other works in the literature ~\cite{gorenflo2020fastfabric,ali2018blockchain} have also focused on a \textit{low-overhead} approach for bootstrapping through block snapshots. This process
is less time-consuming and bypasses most of the steps, but the native snapshot strategies at present are quite
ad-hoc, siloed, and do not have a standardized process of saving historical data.
% Blockchain peers are, in general, personal computers. 
% It is difficult to cope with storage and resource specifications of the updated local copy of all other nodes (or clusters of nodes) 
% ~\cite{carminati2018confidential}. 
% The traditional bootstrapping of a new peer or organization joining the chain ideally needs downloading genesis block, headers, references replaying historical transactions, endorsements, channel version upgrade activities ~\cite{hlfledgersnapshot}, etc.,
% to perform as a peer. 
% The process is considerably long and can easily take days or even weeks, depending on the
% hardware and the network capabilities. 

% \subsection{Interoperability based Approach}
% Recent research and development in decentralized systems has provided many systems that satisfy various functional objectives. However, these are often incompatible to bridge together which has led to the scattering of the blockchains. 
% To pursue interaction between various decentralized systems, such as blockchains, the concept of interoperability has been researched extensively in recent past.
% . Atomic swaps enable users to swap their assets in an atomic and trustless manner
% (i) locking (or extinguishing) of an asset on a source blockchain; (ii) blockchain transfer commitment; and (iii) creation of a representation of the asset on a target blockchain \cite{belchior2022hermes}.
% Atomic swaps are the most reliable solution for asset exchange between parties with zero trust.
% These cross-chain asset transfers rely on an atomic three-phase procedure:
% In the passive phase, a blockchain monitors transactions or events occurring on another blockchain, whereas a blockchain in active mode first sends information to another blockchain and then waits for feedback from that chain. 
% However, an indefinite wait or failure of peer response may create a bottleneck in the proposed feedback mechanism. 
% An alternative approach, such as side-chain-based processing, has also been researched to overcome the drawback of feedback-act-based mechanisms.
% has also been proposed as one of the interoperability areas. 
% It 
% is a trusted third-party solution that comprises an entity called a notary. 
% The notary monitors multiple blockchains and responds upon events triggering interoperable transactions on blockchains 
% which hold keys to verify and sign the transactions \cite{belchior2021survey}. 
% This approach improves fault tolerance but suffers from the dependency on third-party bias.
% have also created a growing interest in research communities. 
% Relay is an application-specific data structure for blockchain interoperability connecting different blockchains. 
% Relays 
% Relays work in parallel with other connected blockchains. When a blockchain connected to the relay chain wants to perform cross-chain operations, it must verify transaction information through the relay chain, which will then transfer
% the information to the target blockchain for blockchain interoperability.
% However, these approaches refer to blockchain networks that are interoperable by initial design and provide the capability for forking new nodes as part of interoperability instead of enabling blockchain interoperability for currently running standalone blockchains and mainly used for cryptographic token exchange. 
% Apart from this, they concentrate more on cryptographic tokens or currency transfers. As a result, these solutions may not be directly applied to pre-existing permissioned blockchains.
% But these existing inter-blockchain communication approaches do significantly detail cross-chain repudiability.

% Abebe \textit{et al.}~\cite{abebe2019enabling}.
% proposed such a relay-based interoperability solution between Hyperledger Fabric networks. 
% We also extended this approach for our cross-network data transfer.
% The traditional bootstrapping of a new peer or organization joining the chain ideally needs downloading genesis block, headers, references replaying historical transactions, endorsements, channel version upgrade activities ~\cite{hlfledgersnapshot}, etc.,
% to perform as a peer. 
% The process is considerably long and can easily take days or even weeks, depending on the
% hardware and the network capabilities. 
% A snapshot is a set of reference markers for the state of data at a given point in time ~\cite{hlf}.






